Anytime Continual Learning for Open Vocabulary Classification

We propose an approach for anytime continual learning (AnytimeCL) for open vocabulary image classification. The AnytimeCL problem aims to break away from batch training and rigid models by requiring that a system can predict any set of labels at any time and efficiently update and improve when receiving one or more training samples at any time. Despite the challenging goal, we achieve substantial improvements over recent methods. We propose a dynamic weighting between predictions of a partially fine-tuned model and a fixed open vocabulary model that enables continual improvement when training samples are available for a subset of a task's labels. We also propose an attention-weighted PCA compression of training features that reduces storage and computation with little impact to model accuracy. Our methods are validated with experiments that test flexibility of learning and inference. Code is available at https://github.com/jessemelpolio/AnytimeCL.

==> figures/latex/data_scenarios.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/data_scenarios.pdf}
\caption{Illustration of continual learning scenarios. Data incremental learning includes seven stages, each comprising 2\%, 4\%, 8\%, 16\%, 32\%, 64\%, and 100\% of task data respectively. Class incremental learning divides a task into five stages, each containing 20\% of classes. In task incremental learning, each task is considered a stage.}
% For data and class incremental scenarios, we run experiments under each target task and average the performances of each stage across different tasks. For task incremental scenario, however, we run through all tasks and treat each task as an individual task.}
\label{fig:data_scenarios}
\end{minipage}
\end{figure}

==> figures/latex/fig2.tex <==
\begin{figure*}[!htb]
 \centering
 \begin{minipage}{\textwidth}
% \includegraphics[width=\linewidth]{figures/incremental_plot.pdf}
\includegraphics[width=\linewidth]{figures/figs/iclr_2024_continual_learning_fig2.pdf}
\caption{\zhen{results figure} (a) Results comparing CLIP zero-shot, TreeProbe (AIM), TreeBlock (AIM) and AnytimeCL (PICE) on target tasks under the data incremental learning scenario. (b) Results of corresponding models on target tasks under class incremental learning. We visualize curves for seen and unseen classes including the overall performance identified with different markers. (c) Results of corresponding models on target tasks under task incremental learning. (d) Flexible inference results after task incremental learning on all tasks.
\label{fig:class_and_task_incremental}
}
\end{minipage}
\end{figure*}

==> figures/latex/fig3.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/iclr_2024_continual_learning_fig3.pdf}
\caption{(a) Results of different complementary models under the task-incremental learning scenario. Numbers included in a bracket are the node capacity of corresponding \tp\ models. (b) We perform an efficiency analysis of \tp\ with different node capacities and \lp\ by estimating how much time needed to incorporate one example into the exemplar model with different number of instances carried in the exemplar set.To minimize randomness, each method is run five times. At each data collection point, we sample an example from the exemplar set and fit it to memory five times. Thus, each data point averages 25 unique simulations. $x$ and $y$-axes are visualized in log scale. (c) The accuracies of different complementary models on target tasks after learning the final stage ($y$-axis) \emph{vs.} the total training time in log scale ($x$-axis).
\label{fig:efficiency_analysis}
}
\end{minipage}
\end{figure}


==> figures/latex/flexible_inference.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/flexible_inference.pdf}
\caption{}
\label{fig:flexible_inference}
\end{minipage}
\end{figure}

==> figures/latex/fusing_operation.tex <==
\begin{figure}[!htb]
 \centering
\begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/fusing_operation.pdf}
\caption{Target (left) and zero-shot (right) accuracies of different fusing operations.}
\label{fig:fusing_operation}
\end{minipage}
\end{figure}


==> figures/latex/incremental_plot.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
% \includegraphics[width=\linewidth]{figures/incremental_plot.pdf}
\includegraphics[width=\linewidth]{figures/OWCL_main_results.pdf}
\caption{Results of various methods. ZS: zero-shot; FT: fine-tune; Exem. Only: only using exemplar-based prediction without considering zero-shot model prediction. (a) Average data incremental results across eight target tasks; (b) Average class incremental results across eight target tasks; (c) Task incremental results on target tasks; (d) Average zero-shot task results across all stages on different continual learning scenarios; (e) Results of flexible inference; (f) Comparison of different fuse operations. Note: for figures (a-d), performances are normalized relative to \czs\ performances on both target and zero-shot tasks. \zhen{Modification ideas after discussion: reorganize (f) to compare AIM and AVG side by side; rotate (d);}
% Dashed red lines in figures (a-c) represent the CLIP results.
% \derek{Can we make memory only --> exemplar only? Add dashed line at 100\% for a,b,c?  Can we put significance bars on (f) and (g)? } \zhen{Finished, except for the significance bar. Update later.}
\label{fig:incremental_plot}
}
\end{minipage}
\end{figure}


==> figures/latex/k_selection.tex <==
\begin{figure}[!htb]
 \centering
% \begin{minipage}{\textwidth}
\includegraphics[width=.6\linewidth]{figures/iclr_knn_methods_and_k_selection.png}
\caption{Results of different versions of KNN on target tasks after finishing all stages under the task incremental learning scenario. We further ablate on $k$ selection so choose $k$ as the $x$-axis. The vertical dashed line represents $k=9$. }
\label{fig:k_selection}
% \end{minipage}
\end{figure}


==> figures/latex/memory_prediction.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/memory_prediction.pdf}
\caption{}
\label{fig:memory_prediction}
\end{minipage}
\end{figure}

==> figures/latex/prompt_tuning.tex <==
\begin{figure}
 \centering
`\includegraphics[width=\linewidth]{figures/figs/prompt_tuning_union_data_incremental.png}
\caption{Ablation of different versions of AnytimeCL-VPT under the union data incremental learning scenario. As an example of naming, ``Shallow (50)'' means the shallow version of AnytimeCL-VPT using 50 learnable visual prompts. 
\label{fig:prompt_tuning}
}
\end{figure}


==> figures/latex/sampling_comparison.tex <==
\begin{figure*}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/figs/sampling_comparison.pdf}
\caption{Comparison of different sampling methods under the union data incremental (a) and class incremental learning (b) scenarios. All methods are trained online. Curves may overlay each other on (b) due to similar performances. Note that no ``past'' classes exist in the first stage of (b). In (b), we plot the accuracy for newly added classes (Current) and for classes seen before the stage began (Past). Note that overall classes include current, past and unseen classes. 
\label{fig:sampling}
}
\end{minipage}
\end{figure*}



==> figures/latex/tree_probe_ensemble_classifier.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/tree_probe_ensemble_classifier.pdf}
\caption{Target and zero-shot task performance comparison w.r.t. ensemble classifiers. ``TreeProbe w/o ensem. cls.'' is the version of TreeProbe by finding the cluster most similar to the input and using the corresponding classifier to predict labels.  The reported accuracy is the average across tasks after incrementally receiving training data from the datasets shown on the $x$-axis.  
% \derek{Should we use normalized accuracy?  Also, the y-axis for the right plot is way too small.}
}
\label{fig:tree_probe_ensemble_classifier}
\end{minipage}
\end{figure}

==> figures/latex/zero_shot_performances.tex <==
\begin{figure}[!htb]
 \centering
 \begin{minipage}{\textwidth}
\includegraphics[width=\linewidth]{figures/zero_shot_performances.pdf}
\caption{Zero-shot performances on data (a), class (b), and task (c) incremental learning scenarios. $x$-axis represents stages when the evaluation is performed.
\label{fig:zero_shot_performances}
}
\end{minipage}
\end{figure}


==> sec/1_introduction_old.tex <==
\section{Introduction}


Our \textbf{anytime continual learning} goal is to receive training examples with {\em any} labels at {\em any} time in {\em any} order and to achieve similar improvements to offline training, while updating efficiently, not requiring additional data, and maintaining zero-shot classification ability. We investigate in the context of open vocabulary image classification. 

Ideally, a learning system should be able to continuously receive samples, update in constant time, and cumulatively improve.  We call this ``anytime continual learning'' and investigate effective mechanisms in the context of open vocabulary image classification.  

Today's foundation models, such as CLIP~\cite{radford_icml2021_clip}, are trained extensively and then frozen and deployed. Given new training data, it is not obvious how to improve them while maintaining their generality and without prohibitively expensive retraining.  While receiving new training samples in a data incremental, class incremental, or task incremental fashion, we aim to continuously improve performance on tasks related to those samples while retaining similar zero-shot ability for arbitrary tasks.  

Our work is most closely related to Zhu \etal.~\cite{treeprobe}, which is inspired by complimentary learning systems theory~\cite{cls_oreilley_2014} and combines a frozen CLIP model and a set of linear models trained on hierarchically clustered data. By limiting the size of the clusters and appropriately weighting the predictions of the two systems, they are able to incorporate a new sample in constant time as the training data grows, improve performance in target tasks, and retain zero-shot and flexible inference ability.  Likewise, our approach combines predictions from a frozen CLIP model and a continually trained model, but we improve on Zhu \etal.'s work in two main ways. 

First, while they freeze the encoder, we improve it by partial fine-tuning, modifying only the last transformer block, which further improves prediction accuracy. We investigate how to best update the fine-tuned model and find that simply training one small-batch iteration per incoming sample with an appropriate learning rate is surprisingly effective. 

Second, we improve the method to weight the systems' predictions. We estimate the relative effectiveness of the zero-shot and fine-tuned representations for each class by computing 1-NN leave-one-out cross-validation on the embeddings from each model.
% We also introduce an ``other'' logit, trained to be the second most confident prediction (besides the correct label), modeling the likelihood that the true class is within the model's range. 
Together, these are used to weight the predictions of the original and fine-tuned models, which is more effective than Zhu \etal.'s method to use the zero-shot classification confidence as a weight.

Since partial fine-tuning requires storing and reprocessing full images or storing the partially encoded representation, we also investigate how to compress the intermediate features. We apply a per-image weighted PCA, which provides a 30x reduction of data with little impact on prediction accuracy.  Such compression could be especially beneficial in a large-scale federated learning setting.

We experiment on the setup of Zhu \etal.~\cite{treeprobe}, which includes data-incremental, class-incremental, and task-incremental learning and evaluation of target task, zero-shot task, and mixed task prediction across several datasets.  %We also experiment on the task-incremental setup from ZSCL~\cite{ZSCL}. 
Our method substantially outperforms prior approaches, while also adding the ability to efficiently incorporate a single example into the model. 

In summary, our contributions follow.
\begin{itemize}
\item Online training: We show the effectiveness of partial fine-tuning as an efficient and effective way to continually improve models from data streams.
\item Complementary systems: We propose an effective weighting method to combine predictions from a frozen open vocabulary model and a continually updating example-based model to enable gaining expertise while maintaining zero- shot ability.
\item Feature compression: We propose a per-image weighted PCA compression of transformer tokens that greatly reduces the storage and computation required for partial fine-tuning with similar prediction accuracy.
\item SotA Performance: In diverse experiments, we demonstrate the effectiveness of these contributions and of the system overall.
\end{itemize}

==> sec/3_method.tex <==
\section{Method}

Our approach is illustrated in Figure~\ref{fig:main_diagram}. We now describe the problem formulation (Sec.~\ref{sec:method_problem}), our multi-model system (Sec.~\ref{sec:method_model}), frequency-weighted sampling (Sec.~\ref{sec:method_sampling}), dynamic class-sensitive prediction weighting (Sec.~\ref{sec:method_weighting}), and weighted per-image PCA feature compression (Sec.~\ref{sec:method_compression}).


\input{figures/latex/main_diagram}

\subsection{Problem formulation}
\label{sec:method_problem}

In open vocabulary image classification, we have a model $f(x, y; \mathbf{\theta})$, parameterized by $\mathbf{\theta}$, that produces a score of assigning image $x$ to label $y$.   %Sequentially, given some new training example(s) $(x_i, y_i)$, our goal is to improve the model's prediction accuracy within limited time. %We call this ``anytime continual learning'' because the model should incorporate new examples, which can arrive in any order, efficiently and effectively without forgetting previously learned tasks.
In our experiments, we start with a publicly available CLIP~\cite{clip} model that has been trained contrastively on image-text pairs. The CLIP model produces a probability for label $y_j$ for image $x_i$ given a set of candidate text labels $\mathcal{Y}$ based on the dot product of image embedding $e_{x_i}$ (CLS token) and text embedding $e_{y_j}$:  
\begin{equation}
\label{eq:class_wise_probability}
    p_z(y=y_j|x_i) = \frac{\exp(100 \cdot \cos(e_{x_i}, e_{y_j}))}{\sum_{y_k\in\mathcal{Y}}^{\mathcal{Y}} \exp(100 \cdot \cos(e_{x_i}, e_{y_k}))}.
\end{equation}

A task is defined by the distribution of images and set of candidate labels $\mathcal{Y}$. Using the setup from~\cite{treeprobe}, we sequentially receive sets of training examples $(\mathbf{x}_i, \mathbf{y}_i)$ for a given task in a {\em data-incremental} (partition of random ordering) or {\em class-incremental} (partition of class-sorted ordering). Or, in a {\em task-incremental} setting, we receive all examples for each task sequentially.  Within each set, we incorporate new examples one by one in an online fashion.  Optionally, we may take a wake/sleep strategy, where after each set is incorporated via online training, the entire model may be further processed offline without receiving new examples.  After receiving each set, the model is evaluated on the entire task (including classes not yet seen in training) for data- or class-incremental, or on all tasks (including tasks not yet seen in training) for task-incremental.  In evaluation, $\mathcal{Y}$ is provided, but there is no other task identifier or indication whether an example's label has been seen in training.  The model should improve on classes for which training examples are received, while retaining the original CLIP model's performance on other classes.  This is evaluated using both the ``target tasks'' (for which training samples are provided) and ``zero-shot tasks'' (for which no training samples are provided) and tasks that are created from a union or mix of target and zero-shot tasks.




%The data stream $\mathcal{D}$ provides infinite annotated instances $(x, y)$ to the model one by one, where $x$ is the image and $y$ is the label. Instances are stored in an exemplar set $\mathcal{E}$ with $i$ being the index in the set. The target of anytime continual learning is to train a model to internalize the incoming instances effectively without much forgetting of learned tasks. 

%We follow the open-vocabulary continual classification setting as Zhu~\etal.~\cite{treeprobe} to incrementally improve performance on target tasks whereas its zero-shot categorization capability is not compromised. We also leverage CLIP~\cite{clip} which is trained to maximize the similarity between images and the corresponding text descriptions. CLIP exhibits compelling zero-shot categorization ability on a wide range of tasks. Specifically, given a test image $x_i$ and the possible candidate text labels $\mathcal{Y} = \{y_j\}_{j \in \{1, \dots, \eta \}}$, CLIP maps them to the corresponding image embedding $e_{x_i}$ and text embeddings $\{e_{y_j}\}_{j \in \{1, \dots, \eta \}}$ through the image encoder and text encoder:
%\begin{equation}
%    e_{x_i} = \mathbf{F}_{\text{img}}(x_i), \quad e_{y_j} = \mathbf{F}_{\text{txt}}(y_j).
%\end{equation}
%Then the class-wise probability of the image being label $y_j$ is:
%\begin{equation}
%\label{eq:class_wise_probability}
%    p_z(y=y_j|x) = \frac{\exp(\tau \cdot \cos(e_{x_i}, e_{y_j}))}{\sum_r^{\eta} \exp(\tau \cdot \cos(e_{x_i}, e_{y_r})) },
%\end{equation}
%where the temperature parameter $\tau$ is set to 100 in CLIP and $\cos$ computes the cosine similarity between two input vectors.

\subsection{Model Overview}
\label{sec:method_model}

Similar to Zhu \etal~\cite{treeprobe}, we use complementary models to retain zero-shot performance while improving in the target tasks. One model is the unchanged CLIP model, and the second ``exemplar'' model is trained on the provided examples. Zhu \etal~\cite{treeprobe} use a linear classifier on the CLIP CLS token output for the exemplar model, which can be trained quickly. They further use a binary tree clustering to partition the training data into nodes containing a limited number of examples and train linear classifiers in each leaf node, providing controllable constant time training with small loss in prediction accuracy. However, their model's capacity to improve is limited by not fine-tuning the earlier layers, and the linear classifier can still take several seconds to train, even with small training nodes.

Instead, we propose to partially fine-tune the last layer(s) while maintaining a copy of the original.  Prediction can then be performed with the original CLIP parameters $\mathbf{\theta}\in\{\mathbf{\theta}_b,\mathbf{\theta}_0\}$ or tuned parameters as $\mathbf{\theta}\in\{\mathbf{\theta}_b,\mathbf{\theta}_{ft}\}$, where $\mathbf{\theta}_b$ are the shared parameters, $\mathbf{\theta}_0$ the original parameters of the last layer(s), and  $\mathbf{\theta}_{ft}$ are the tuned parameters.  Our experiments use the the ViT version~\cite{ViT} of CLIP, and we tune only the last transformer block.  Training more blocks provides quickly diminishing returns at greater cost~\cite{CLIPItself}. The tuned model produces an image embedding (CLS token) that is dot-multiplied with the frozen CLIP text embedding of each label to produce the label score.

As in~\cite{treeprobe}, the final probability is a weighted average of both models' outputs:
\begin{equation}
    \begin{split}
        p_{\text{out}}(y=y_j|x_i) &= \alpha(x_i,y_j) p_{\text{tar}}(y=y_j|x_i) \\
    &+ (1 - \alpha(x_i,y_j)) p_{\text{zs}}(y=y_j|x_i),
    \end{split}
\end{equation}
where $p_{\text{tar}}$ is the output of the fine-tuned exemplar model (trained to predict on target classes/tasks), $p_{\text{zs}}$ is the output of the original CLIP model (capable of zero-shot prediction over any label set), and $\alpha(x_i,y_j)$ is a weighting based on relative applicability and effectiveness, which we call the {\em Dynamic Class-sensitive Weighting (DCW)}. 

\subsection{Online Training}
\label{sec:method_sampling}

Recent broad evaluations~\cite{prabhu_gdumb_eccv_2020,prabhu_budgetedCL_cvpr_2023} show that, given either a storage or computational budget, simple replay strategies work best. Common strategies include first-in-first-out (FIFO), where the most recently received samples are trained for some number of iterations, uniform random sampling in each batch, or class-balanced (``ring buffer'') sampling in each batch.  FIFO suffers from continual domain shift and forgets earlier examples.  Uniform or class-balanced sampling from all training samples does not sufficiently incorporate the more recently received samples without many iterations of training.  

To overcome these problems, we propose a simple strategy that we call {\bf Frequency Weighted Sampling} (FWS). When a new sample $x_i$ is received, its sampling weight $w_i$ is initialized to 1. After including the sample in a training batch, the weight is updated by:
\begin{equation}
    w_i=\max(w_i * \xi, w_{\min}),
\end{equation}
where $\xi \in [0, 1]$ is the decay multiplier. $\xi$ adjusts the degree of frequency bias---larger values lead to more repeated sampling of recently added examples.  To be clear, $w_i$ is proportional to the likelihood that a training sample is used in the next training batch, not as a loss weight.  We set a lower bound $w_{\min}$ for sampling weights, for numerical stability and to ensure relatively well-trained instances have equal chance of being sampled.  When a new training example is received, a batch of size $B$ is filled with that example and $B-1$ other random stored examples, drawn with a $w_i$ weighting. One training iteration is performed with that batch. The FWS strategy hastens convergence to the expectation that all training samples are eventually sampled an equal number of times, regardless of their order of appearance. 

FWS works well, but we find that uniform random sampling and class-balanced sampling perform similarly, as long as appropriate learning rates are used.  %We use a batch size of 32 with a learning rate of (32/2048)*1e-4 and find that scaling them up proportionally can also work well but with higher computational cost. 

\subsection{Dynamic Class-sensitive Weighting}
\label{sec:method_weighting}

The prediction weighting $\alpha(x_i,y_j)$ should encode whether the example $x_i$ likely falls into the label range of the exemplar model and the relative accuracy of the exemplar and original CLIP models for label $y_j$. This is not fully captured by Zhu~\etal.~\cite{treeprobe} that compute $\alpha(x_i,y_j)$ as the total probability, according to $p_\text{zs}(y_j|x_i)$ that $y_j\in\mathcal{Y}$ is in the set of training labels, since this makes $\alpha$ independent of the exemplar model and of the label $y_i$.   

We compute $\alpha(x_i,y_j)$ as follows:
\begin{equation}
    \label{eq:final_alpha}
    \alpha(x_i,y_j)= \frac{(1-p_{\text{other}}(x_i))c_\text{tar}(y_k)}{(1-p_{\text{other}}(x_i)) c_\text{tar}(y_k) + c_\text{zs}(y_k) + \epsilon}.
\end{equation}
$(1-p_{\text{other}})$ is the estimated probability that an example falls outside the exemplar model range.  $c_\text{tar}$ and $c_\text{zs}$ are the estimated accuracy of each model for the label $y_j$. $\epsilon$ is a very small number (1e-8) to prevent division by zero.

In experiments, we find that the $p_{\text{other}}$ term is somewhat effective on its own but does not significantly improve over using only the $c_\text{tar}$ and $c_\text{zs}$ terms. We include description because it is used in our experiments and may be more useful in other contexts.

\vspace{2mm} \noindent {\bf The ``Other'' Class Prediction}.  Predicting whether an example's label is within a model's range is challenging, particularly as we do not want to use external data or complex processes.  Our idea is to require in training that the true label has a much higher score than incorrect labels and an ``other'' label (via softmax cross-entropy), and that the ``other'' label has higher score than the incorrect labels.  In other words, the true label should score highest if known, but otherwise ``other'' should score highest. To avoid overfitting to the training samples, the score for the ``other'' label is a single learned logit value that does not depend on the input.

The combined loss is: 
\begin{equation}
\begin{split}
    \mathcal{L}(x_i, y_i, \mathcal{Y}) = & \mathcal{L}_{\text{ce}}(x_i,y_i,\mathcal{Y} \cup \text{other}) + \\ 
    & \beta \mathcal{L}_{\text{ce}}(x_i,\text{other},(\mathcal{Y} \cup \text{other}) \setminus y_i)
\end{split}
\end{equation}
where $y_i$ is the true label and $\mathcal{L}_{\text{ce}}(x, z, \mathcal{Z})$ is the cross-entropy loss when the true label is $z$ and the label space is $\mathcal{Z}$.  $\beta$ is a hyperparameter, set to $0.1$ based on validation experiments. 

\vspace{2mm} \noindent {\bf Per-class Confidence Estimation}.  The tuned and original model may have different relative accuracies for different labels within the exemplar model's range.  To account for this, the accuracy of each model for each label is estimated using leave-one-out nearest neighbor cross-validation. $c_{\text{tar}}(y_j)$ is estimated using the CLS embedding from the fine-tuned model, and $c_{\text{zs}}(y_j)$ is estimated using the CLS embedding from the original CLIP model.  In both cases, the cross-validation accuracy is measured for class $y_j$ using currently received training samples and cosine distance.  
If there are one or fewer examples with label $y_j$ in the training examples, then $\alpha(x_i,y_j)=0$. If all labels in $\mathcal Y$ are present in the training examples, we set $\alpha(x_i,y_j)=1$.

Using cross-validation to compute $c_{\text{tar}}(y_j)$ is more robust than confidence over training examples, since the exemplar model has fit to the training examples.  We also experimented with setting $c_{\text{zs}}(y_j) = p_\text{zs}(y_j|x_i)$, which slightly worse results, perhaps because that method uses different bases of comparison for the two models.  

When training and inference are concurrent, the computation of $c_{\text{tar}}(y_j)$ and $c_{\text{zs}}(y_j)$ can be made more efficient by caching distances and less frequently updating the embeddings used for nearest neighbor calculation.  A fast alternative is to estimate the accuracy for each class using an exponential moving average of the true class probability as training examples are received for both the original and fine-tuned model.

% we denote each exemplar in class $y_i$ as $e_{y_i}^j$ where $j$ is the exemplar index and the number of exemplars of this class is denoted by $N_{y_i}$. We retrieve two most similar exemplars in the node and leave out the most similar exemplar since it literally would be the query image embedding. Assuming that the corresponding label of the retrieved sample is $\hat{y}^j$, we calculate the accuracy of this class as $\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$ and this is the probability of $p_{\text{ft}}(y_i)=\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$.

% $\mathbf{M}_{\text{ft}}$ 

% Since $\mathbf{M}_{\text{ft}}$ is directly fine-tuned on target tasks, it has better performance on classes from target tasks whereas $\mathbf{M}_{\text{zs}}$ is more trustworthy in other classes. Therefore, selecting a proper model for making the prediction is vital to the overall performance. Zhu \etal.~\cite{treeprobe} relies on the confidence of $\mathbf{M}_{\text{zs}}$ on  exemplar classes

% Our method extends upon TreeProbe~\cite{treeprobe}, which fits data into a hierarchical tree and train a linear classifier within each leaf node. 


% Let $\mathcal{M}_{\text{ft}}$ the nearest fine-tuned model, $\mathcal{M}_{\text{zs}}$ the zero-shot model. Assume the node of the fine-tuned model has $\mathcal{N}$ exemplars, $\mathcal{C}_e$ classes, and the label for each class is $y_i, 1\le i \le \mathcal{C}_e$. During inference, we use $\mathcal{C}_t$ to represent the number of target classes.

% For $\mathcal{M}_{\text{ft}}$, we first encode the intermediate features of each exemplar in the node using the fine-tuned weights. We then iterate all classes in the node and compute the leave-one-out retrieval accuracies for all classes. 

% Specifically, we denote each exemplar in class $y_i$ as $e_{y_i}^j$ where $j$ is the exemplar index and the number of exemplars of this class is denoted by $N_{y_i}$. We retrieve two most similar exemplars in the node and leave out the most similar exemplar since it literally would be the query image embedding. Assuming that the corresponding label of the retrieved sample is $\hat{y}^j$, we calculate the accuracy of this class as $\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$ and this is the probability of $p_{\text{ft}}(y_i)=\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$. Afterwards, we map $p_{\text{ft}}$ to the target classes by multiplying an affinity mask of shape $\mathcal{C}_e \times \mathcal{C}_t$, where 1 indicates an overlapping class in both target and exemplar class sets, and 0 elsewhere. The size of $p_{\text{ft}}$ for each instance is $\mathcal{C}_t$, the number of target classes. 

% Regarding the zero-shot confidence $p_{\text{zs}}$, it shares the same calculation procedure but we use the encoded representations from the zero-shot transformer block for retrieval. 







% Assuming the logit for the other class is denoted as $l_{\text{other}}$, the encoded image embedding is $e_{\text{ft}}^I$, and the text embedding for target class $y_t$ is $e_{y_t}$, then
% \begin{equation}
% \label{eq:p_other}
%     p_{\text{other}} = \frac{\exp({l_{\text{other}}})}{\sum_{y_t}^{\mathcal{C}_t} \exp({100 * e_{\text{ft}}^I e_{y_t}}) + \exp({l_{\text{other}}})}.
% \end{equation}

% We are inspired by the open-world recognition literature~\cite{??} to introduce the prediction of an ``other'' class. If a sample is assigned to the other class, it means that the sample is OOD. The success of predicting an OOD sample as the other class is mainly practiced by drawing negative samples as learning materials to help the model discern the boundary between the ``other'' class and all other classes. 


% Then the $\alpha$ is calculated by:
% \begin{equation}
%     \alpha = (1-\sigma p_{\text{other}})(\frac{p_{\text{ft}}}{p_{\text{ft}} + p_{\text{zs}}  + \epsilon}).
% \end{equation}
% Here, $\epsilon=1e^{-6}$ is used to avoid cases where the divisor is 0.  

% Then the final probability of our system is:
% \begin{equation}
%     p_{\text{out}} = \alpha p_e + (1-\alpha) p_z,
% \end{equation}
% here $p_e=\text{softmax}(100 * e_{\text{ft}}^I e_{y_t})$ and $p_z = \text{softmax}(100 * e_{\text{zs}}^I e_{y_t})$. $e_{\text{zs}}^I$ is the encoded image embedding from the zero-shot transformer block.



\subsection{Storage efficiency and privacy}
\label{sec:method_compression}

Partial tuning of our models requires either storing each image or storing the features (or tokens) that feed into the tuned portion of the model. Storing images is disadvantageous in terms of privacy, storage of the full model and images, and in requiring full processing of the images at each iteration. Storing features alleviates some of these problems, but still uses much memory or storage.  Therefore, we investigate how to compress the training features, aiming to increase storage and computational efficiency while maintaining training effectiveness. The compressed features also provide more privacy than storing original images, though we do not investigate how well the images can be recovered from compressed features.

Well-trained networks learn data-efficient representations that are difficult to compress. Indeed, if we try to compress feature vectors with VQ-VAE~\cite{vqvae_neurips2027_van_oord} or PCA~\cite{Pearson_PCA_1901} trained on a dataset, we are not able to achieve any meaningful compression without great loss in training performance. The features within {\em each image}, however, contain many redundancies. We, therefore, compute PCA vectors on the features in each image and store those vectors along with the coefficients of each feature vector. Further, not all features are equally important for prediction. We, therefore, train a per-image attention-weighted PCA, weighted by attention between each token and the CLS token. Finally, we can compress further by storing min/max floating point values for each vector and for the coefficients and quantizing them to 8-bit or 16-bit unsigned integers. See the supplemental material for details.  By storing only five PCA vectors and their coefficients this way, we can reduce the storage of fifty 768-dim training patch tokens from 153K bytes to 5K bytes with less than 1\% difference in prediction accuracy. 

==> sec/backup0_3_method.tex <==
\section{Method}

\subsection{Problem formulation}

In open vocabulary image classification, we have a model $f(x, y, \mathcal{Y}; \mathbf{\theta})$, parameterized by $\mathbf{\theta}$, that produces a score of assigning image $x$ to label $y$ given candidate labels $\mathcal{Y}$. A task is defined by the distribution of images and candidate labels.  Sequentially, given some new training example(s) $(x_{tr}, y_{tr})$, our goal is to improve the model's prediction accuracy within limited time. %We call this ``anytime continual learning'' because the model should incorporate new examples, which can arrive in any order, efficiently and effectively without forgetting previously learned tasks.

In our experiments, we start with a publicly available CLIP~\cite{clip} model that has been trained contrastively on image-text pairs. The CLIP model produces a probability for label $y_j$ for image $x_i$ given a set of text labels $\mathcal{Y}$ based on the dot product of image embedding $e_{x_i}$ and text embedding $e_{y_j}$:.  
\begin{equation}
\label{eq:class_wise_probability}
    p_z(y=y_j|x_i) = \frac{\exp(100 \cdot \cos(e_{x_i}, e_{y_j}))}{\sum_{y_k\in\mathcal{Y}}^{\mathcal{Y}} \exp(100 \cdot \cos(e_{x_i}, e_{y_k}))}.
\end{equation}

In experiments, using the setup from~\cite{treeprobe} we may sequentially receive sets of training examples for a given task in a data-incremental (partition of random ordering) or class-incremental (partition of class-sorted ordering). Or, in a task-incremental setting, we receive all examples for each task sequentially.  Within each set, we incorporate new examples one by one in an online fashion.  Optionally, we may take a wake/sleep strategy, where after each set is incorporated via online training, the entire model may be further processed offline without receiving new examples.  After receiving each set, the model is evaluated on the entire task (i.e. all classes including any not yet seen in training) for data- or class-incremental, or on all tasks (including tasks not yet seen in training) for task-incremental.  In evaluation, neither task identifier nor indication of whether an example's label is seen in training is provided.  The model should improve on classes for which training examples are received, while retaining the original CLIP model's performance on other classes.  This is evaluated using both the ``target tasks'' (for which training samples are provided) and ``zero-shot tasks'' (for which no training samples are provided).

Ultimately, the goal is to receive any training examples at any time in any order and to achieve similar improvements to offline training, while updating efficiently, not requiring additional data, and maintaining the original CLIP model's zero-shot ability.  We call this ``anytime continual learning''.  


%The data stream $\mathcal{D}$ provides infinite annotated instances $(x, y)$ to the model one by one, where $x$ is the image and $y$ is the label. Instances are stored in an exemplar set $\mathcal{E}$ with $i$ being the index in the set. The target of anytime continual learning is to train a model to internalize the incoming instances effectively without much forgetting of learned tasks. 

%We follow the open-vocabulary continual classification setting as Zhu~\etal.~\cite{treeprobe} to incrementally improve performance on target tasks whereas its zero-shot categorization capability is not compromised. We also leverage CLIP~\cite{clip} which is trained to maximize the similarity between images and the corresponding text descriptions. CLIP exhibits compelling zero-shot categorization ability on a wide range of tasks. Specifically, given a test image $x_i$ and the possible candidate text labels $\mathcal{Y} = \{y_j\}_{j \in \{1, \dots, \eta \}}$, CLIP maps them to the corresponding image embedding $e_{x_i}$ and text embeddings $\{e_{y_j}\}_{j \in \{1, \dots, \eta \}}$ through the image encoder and text encoder:
%\begin{equation}
%    e_{x_i} = \mathbf{F}_{\text{img}}(x_i), \quad e_{y_j} = \mathbf{F}_{\text{txt}}(y_j).
%\end{equation}
%Then the class-wise probability of the image being label $y_j$ is:
%\begin{equation}
%\label{eq:class_wise_probability}
%    p_z(y=y_j|x) = \frac{\exp(\tau \cdot \cos(e_{x_i}, e_{y_j}))}{\sum_r^{\eta} \exp(\tau \cdot \cos(e_{x_i}, e_{y_r})) },
%\end{equation}
%where the temperature parameter $\tau$ is set to 100 in CLIP and $\cos$ computes the cosine similarity between two input vectors.

\subsection{Model Overview}

Similar to Zhu \etal~\cite{treeprobe}, we use complementary models to retain zero-shot performance while improving in the target tasks. One model is the unchanged CLIP model, and the second ``exemplar'' model is trained on the provided examples. Zhu \etal~\cite{treeprobe} use a linear classifier on the CLIP CLS token output for the exemplar model, which can be trained quickly. They further use a binary tree clustering to partition the training data into nodes containing a limited number of examples and train linear classifiers in each leaf node, providing controllable constant time training with small loss in prediction accuracy. However, their model's capacity to improve is limited by not fine-tuning the earlier layers.

Instead, we propose to partially fine-tune the last layer(s) while maintaining a copy of the original.  Prediction can then be performed with the original CLIP parameters $\mathbf{\theta}\in\{\mathbf{\theta}_b,\mathbf{\theta}_0\}$ or tuned parameters as $\mathbf{\theta}\in\{\mathbf{\theta}_b,\mathbf{\theta}_{ft}\}$, where $\mathbf{\theta}_b$ are the shared parameters, $\mathbf{\theta}_0\}$ the original parameters of the last layer(s), and  $\mathbf{\theta}_{ft}$ are the tuned parameters.  Our experiments use the the ViT version~\cite{ViT} of CLIP, and we tune only the last transformer block.  Training more blocks provides quickly diminishing returns at greater cost. 

\subsection{Exemplar Model Online Training}

Recent broad evaluations~\cite{prabhu_gdumb_eccv_2020,budgetedCL} show that, given either a storage or computational budget, simple replay strategies work best. Common strategies include first-in-first-out (FIFO), where the most recently received samples are trained for some number of iterations, uniform random sampling in each batch, or class-balanced (``ring'') sampling in each batch.  FIFO suffers from continual domain shift and forgets earlier examples.  Uniform or class-balanced sampling from all training samples does not sufficiently incorporate the more recently received samples without many iterations of training.  

To overcome these problems, we propose a remarkably simple and effective sampling strategy that we call Recency Weighted Sampling.  When a new sample $x_i$ is received, its sampling weight $w_i$ is initialized to 1. Afterwards, the weight is updated by:
\begin{equation}
    w_i=\max(\xi^{T_i}, w_{\min}),
\end{equation}
where $0< \xi <1$ is the decay multiplier and $T_i$ is the number of training iterations that include $x_i$. $\xi$ adjusts the degree of recency bias---larger values lead to more repeated sampling of recent samples.  We set a lower bound for sampling weights, for numerical stability and to ensure relatively old instances have equal chance of being sampled. Our strategy also provides a theoretical guarantee that all training examples are eventually expected to be sampled an equal number of times, regardless of their order of appearance. 

The data stream injects data points to the accumulated data pool one at a time. With new samples placed into the pool, a simple approach to ensure good performance on all learned tasks is to iteratively train the model all accumulated data points. But this approach quickly becomes computationally infeasible when the pool is large. To keep a constant learning speed, we only assign one batch of training where the batch must contain the incoming sample with others drawn from the pool. However, once joining the pool, the new sample easily disperses, leading to ineffective learning on new data points. 

To mitigate this problem, we develop a Recency Weighted Sampling strategy to assign higher weights for more recent data points. 
At the time a new sample $x_i$ is received, its initial sampling weight $\mathcal{W}_{x_i}$ is set 1. Afterwards, the weight is updated by:
\begin{equation}
    \mathcal{W}_{x_i}=\max(\xi^{T_{x_i}}, \mathcal{W}_{\min}),
\end{equation}
where we call $0< \xi <1$ the decay multiplier and $T_{x_i}$ is the number of iterations of $x_i$ seen by the model. $\xi$ adjusts the degree of recency bias---larger values extend the stay of newer samples in batches. We set a lower bound for sampling weights, to ensure relatively old instances have equal chances to be sampled. Our strategy also provides a theoretical guarantee that all data points in the pool are sampled an equal amount of times in the long run.


%Zhu \etal~\cite{treeprobe} chose to freeze the image encoder while building linear classifiers in leaf nodes of a hierarchy tree on top of image embeddings. This can be limiting in the performance on some target tasks since the final image embeddings may overlook some information beneficial to the task. Inspired by the idea of building a side car network~\cite{sidetuning} effecitive in task incremental learning, we build a replica of the final layer in the ViT version~\cite{ViT} image encoder and place the replicated layer in parallel with the original layer. We only fine-tune this replicated layer for all of our target tasks. We denote the shared part, the original last layer and the replicated fine-tuned layer as $\mathbf{M}_{\text{base}}$, $\mathbf{M}_{\text{zs}}$, and $\mathbf{M}_{\text{ft}}$\footnote{For simplicity, we call $\mathbf{M}_{\text{base}}$, $\mathbf{M}_{\text{zs}}$, and $\mathbf{M}_{\text{ft}}$ the base model, the zero-shot model, and the fine-tuned model}. Note one can choose to fine-tune more layers for better performance with a compromise in training speed and more demands on the hardware.

% and  while keeping the original image encoder frozen. 
 
% performs zero-shot categorization by mapping the testing image and candidate text labels to corresponding image embedding and text embeddings and calculate the similarities of two modalities. an image $x_i$ to the image embedding $e_{x_i}$ and the candidate textual labels $\mathcal{Y} = \{y_j\}_{j \in \{1, \dots, \eta \}}$ to the text embeddings $\{ e_{y_j}\}_{j \in \{1, \dots, \eta \}}$. 

% Given a target task $\mathcal{T}$ containing a set of textual classes denoted by $\mathcal{C}_t$, 

% Instead of fixing CLIP encoders, we partially fine-tune the last layer ($\mathcal{M}_{\text{zs}}$) of ViT-B/32~\cite{ViT} on accumulated data, which derives the fine-tuned layer denoted by $\mathcal{M}_{\text{ft}}$. 


% \subsection{Pre-requisite}
% \zhen{Introduce open-vocabulary continual learning and TreeProbe}

% \zhen{A diagram figure that shows a pivotal node representing the zero-shot model, and then a tree of several nodes with several images of different categories. The input image is a cat and then it finds a nearest node with the cat category. The output from that node model and the pivotal model are aggregated through a PICE module.}

% Given an open-vocabulary classification model, open-vocabulary continual learning aims to bring consistent improvements for target tasks


% \subsection{AnytimeCL}

\input{figures/latex/main_diagram}

As shown in Fig.~\ref{fig:main_diagram}, the image is first fed to the base model $\mathbf{M}_{\text{base}}$ to get an intermediate representation $e_{\text{mid}}$. Then $e_{\text{mid}}$ is processed by the parallel $\mathbf{M}_{\text{zs}}$ and $\mathbf{M}_{\text{ft}}$, respectively. The output of $\mathbf{M}_{\text{zs}}$ is exactly the image embedding and therefore its probabilistic prediction given the candidate labels is $p_{z}(y=y_j|x)$. Likewise, $\mathbf{M}_{\text{ft}}$ produces a fine-tuned image embedding and then the probabilistic output can be computed through Eq.~\ref{eq:class_wise_probability}, which we denoted as $p_{\text{ft}}(y=y_j|x)$. Like in~\cite{treeprobe}, the final probability is composed by both probabilities:
\begin{equation}
    p_{\text{out}}(y=y_j|x) = \alpha p_{\text{ft}}(y=y_j|x) + (1 - \alpha) p_{\text{zs}}(y=y_j|x),
\end{equation}
here $\alpha$ represents the confidence of the fine-tuned model of its prediction.

\subsection{Online learning}
The data stream injects data points to the accumulated data pool one at a time. With new samples placed into the pool, a simple approach to ensure good performance on all learned tasks is to iteratively train the model all accumulated data points. But this approach quickly becomes computationally infeasible when the pool is large. To keep a constant learning speed, we only assign one batch of training where the batch must contain the incoming sample with others drawn from the pool. However, once joining the pool, the new sample easily disperses, leading to ineffective learning on new data points. 

To mitigate this problem, we develop a Recency Weighted Sampling strategy to assign higher weights for more recent data points. 
At the time a new sample $x_i$ is received, its initial sampling weight $\mathcal{W}_{x_i}$ is set 1. Afterwards, the weight is updated by:
\begin{equation}
    \mathcal{W}_{x_i}=\max(\xi^{T_{x_i}}, \mathcal{W}_{\min}),
\end{equation}
where we call $0< \xi <1$ the decay multiplier and $T_{x_i}$ is the number of iterations of $x_i$ seen by the model. $\xi$ adjusts the degree of recency bias---larger values extend the stay of newer samples in batches. We set a lower bound for sampling weights, to ensure relatively old instances have equal chances to be sampled. Our strategy also provides a theoretical guarantee that all data points in the pool are sampled an equal amount of times in the long run.


\subsection{PICE}

Naively setting $\alpha$ to a static number does not conform to the real case: $\mathbf{M}_{\text{ft}}$ is more confident for classes it is tuned on, and $\mathbf{M}_{\text{zs}}$ is more trustworthy in other classes.
A better alternative is the AIM (adaptive instance marginalization) developed by Zhu~\etal.~\cite{treeprobe}, where $\alpha$ is calculated by summing up the probabilities predicted by the zero-shot model for overlapping classes between the exemplar set and the candidate labels. This approach, however, overlooks the continual increase of the trustfulness of $\mathbf{M}_{\text{ft}}$ on exemplar classes overtime. As a result, we are inspired to search for an $\alpha$ prediction method that counts in the confidence of both models. We hold an intuition that $\alpha$ should be a class-wise estimate, since some classes in the exemplar set may be out-numbered by others and their confidences should not be entirely the same. 

\vspace{2mm} \noindent {\bf Per-class Confidence Estimation.}~For each exemplar class $y_k \in \mathcal{Y}_{e}$, we treat its leave-one-out nearest neighbor accuracy as the class confidence $\mathbf{C}_{\text{ft}}(y_k)$ of $\mathbf{M}_{\text{ft}}$. Let assume $\mathcal{E}_{y_k}$ all exemplars of class $y_k$ in the exemplar set. For each exemplar $\mathcal{E}_{y_k}^i$, we retrieve the most similar exemplar through cosine similarities of the fine-tuned embeddings between $\mathcal{E}_{y_k}^i$ and all other exemplars in the whole exemplar set $\mathcal{E}$:
\begin{equation}
\label{eq:nn_find}
\text{NN}(\mathcal{E}_{y_k}^i) = \argmax_{j \in \mathcal{E} \setminus {i}} \\ \cos(\mathbf{M}_{\text{ft}}(e_{\text{mid}}^i), \mathbf{M}_{\text{ft}}(e_{\text{mid}}^j)).
\end{equation}
Assume $\hat{y}^{i}$ is the label of $\text{NN}(\mathcal{E}_{y_k}^i)$, then:
\begin{equation}
    \mathbf{C}_{\text{ft}}(y_k) = \sum_{i=1}^{|\mathcal{E}_{y_k}|} \frac{\mathds{1}(\hat{y}^i=y_k)}{|\mathcal{E}_{y_k}|},
\end{equation}
where $|\cdot|$ is the set length. Compared to using the model prediction accuracy calculated by taking the prediction as the label with the largest predicted probability, this estimation is more comprehensive as the model prediction accuracy can be 100\% if the model overfits whereas NN is more robust. The per-class confidence $\mathbf{C}_{\text{zs}}(y_k)$ of the zero-shot model can be estimated similarly by substituting $\mathbf{M}_{\text{ft}}$ with $\mathbf{M}_{\text{zs}}$ in Eq.~\ref{eq:nn_find}. After deriving $\mathbf{C}_{\text{ft}}(y_k)$ and $\mathbf{C}_{\text{zs}}(y_k)$, we set
\begin{equation}
\label{eq:initial_alpha}
    \alpha (y_k)= \frac{\mathbf{C}_{\text{ft}}(y_k)}{ \mathbf{C}_{\text{ft}}(y_k) + \mathbf{C}_{\text{zs}}(y_k) },
\end{equation} which means that if $\mathbf{C}_{\text{ft}}(y_k)$ is larger, we give more weight to the fine-tuned model and vice-versa. Note Eq.~\ref{eq:initial_alpha} defines $\alpha$ for an exemplar class. If one candidate class does not appear in the exemplar set, simply $\alpha=0$.

% we denote each exemplar in class $y_i$ as $e_{y_i}^j$ where $j$ is the exemplar index and the number of exemplars of this class is denoted by $N_{y_i}$. We retrieve two most similar exemplars in the node and leave out the most similar exemplar since it literally would be the query image embedding. Assuming that the corresponding label of the retrieved sample is $\hat{y}^j$, we calculate the accuracy of this class as $\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$ and this is the probability of $p_{\text{ft}}(y_i)=\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$.

% $\mathbf{M}_{\text{ft}}$ 

% Since $\mathbf{M}_{\text{ft}}$ is directly fine-tuned on target tasks, it has better performance on classes from target tasks whereas $\mathbf{M}_{\text{zs}}$ is more trustworthy in other classes. Therefore, selecting a proper model for making the prediction is vital to the overall performance. Zhu \etal.~\cite{treeprobe} relies on the confidence of $\mathbf{M}_{\text{zs}}$ on  exemplar classes

% Our method extends upon TreeProbe~\cite{treeprobe}, which fits data into a hierarchical tree and train a linear classifier within each leaf node. 


% Let $\mathcal{M}_{\text{ft}}$ the nearest fine-tuned model, $\mathcal{M}_{\text{zs}}$ the zero-shot model. Assume the node of the fine-tuned model has $\mathcal{N}$ exemplars, $\mathcal{C}_e$ classes, and the label for each class is $y_i, 1\le i \le \mathcal{C}_e$. During inference, we use $\mathcal{C}_t$ to represent the number of target classes.

% For $\mathcal{M}_{\text{ft}}$, we first encode the intermediate features of each exemplar in the node using the fine-tuned weights. We then iterate all classes in the node and compute the leave-one-out retrieval accuracies for all classes. 

% Specifically, we denote each exemplar in class $y_i$ as $e_{y_i}^j$ where $j$ is the exemplar index and the number of exemplars of this class is denoted by $N_{y_i}$. We retrieve two most similar exemplars in the node and leave out the most similar exemplar since it literally would be the query image embedding. Assuming that the corresponding label of the retrieved sample is $\hat{y}^j$, we calculate the accuracy of this class as $\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$ and this is the probability of $p_{\text{ft}}(y_i)=\sum_{j=1}^{N_{y_i}} \frac{\mathds{1}(\hat{y}^j=y_i)}{\mathcal{N}}$. Afterwards, we map $p_{\text{ft}}$ to the target classes by multiplying an affinity mask of shape $\mathcal{C}_e \times \mathcal{C}_t$, where 1 indicates an overlapping class in both target and exemplar class sets, and 0 elsewhere. The size of $p_{\text{ft}}$ for each instance is $\mathcal{C}_t$, the number of target classes. 

% Regarding the zero-shot confidence $p_{\text{zs}}$, it shares the same calculation procedure but we use the encoded representations from the zero-shot transformer block for retrieval. 





\vspace{2mm} \noindent {\bf The ``Other'' Class Prediction.}~Another problem of the above method is with more fine-tuning of the same data, $\mathbf{C}_{\text{ft}}(y_k)$ eventually should be larger than $\mathbf{C}_{\text{zs}}(y_k)$ in every class. This is because $\mathbf{C}_{\text{zs}}(y_k)$ is fixed if no new exemplars are added in whereas $\mathbf{C}_{\text{ft}}(y_k)$ increases. This shall make the model favor the fine-tuned model for every prediction, making the zero-shot model never chosen even for non-exemplar classes. As a result, it is important to further decide the probability of the input sample resides out of domain (OOD).

% \footnote{Out of domain (OOD) means the class of the input sample is never seen by the fine-tuned model}. 

Our idea is to have a standalone logit that can be used to compute the probability of the input sample to be OOD. Suppose this logit is denoted by $l_{\text{other}}$, the probability of the other class is estimated by:
\begin{equation}
\label{eq:p_other}
    p_{\text{other}} = \frac{\exp({l_{\text{other}}})}{\sum_r^{\eta} \exp(\tau \cdot \cos(e_{x_i}, e_{y_r})) + \exp({l_{\text{other}}})}.
\end{equation}

Taking Eq.~\ref{eq:p_other} to Eq.~\ref{eq:initial_alpha}, the modified $\alpha (y_k)$ that discerns the domain gap is defined as:
\begin{equation}
    \label{eq:final_alpha}
    \alpha (y_k)= \frac{(1-p_{\text{other}})\mathbf{C}_{\text{ft}}(y_k)}{(1-p_{\text{other}}) \mathbf{C}_{\text{ft}}(y_k) + \mathbf{C}_{\text{zs}}(y_k) }.
\end{equation}

\vspace{2mm} \noindent {\bf Training Losses For ``Other''.}~Leveraging the probability for ``other'' classes is in a similar spirit to the convention in the open-world recognition literature~\cite{??} where the ``other'' class is used to identify samples requiring further processing or annotation. In most approaches, their setups allow using out-of-domain data to facilitate the training of the ``other'' logit. By incorporating those OOD data, they can leverage normal cross-entropy loss to train all target classes including the ``other'' class. 
However, since all of our training materials come from the exemplar set, we cannot enforce the same practice. 

Instead, we introduce an additional loss term that favors the ``other'' class as the second most confident prediction besides the correct class. Specifically, the fine-tuned model is trained with the following loss function:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{\text{ce}}(y_{\text{correct}}; \mathcal{Y} \cup l_{\text{other}} ) + \beta \mathcal{L}_{\text{ce}} (l_{\text{other}}; \mathcal{Y} \setminus y_{\text{correct}} \cup l_{\text{other}} ).
\end{equation}
$\mathcal{L}_{\text{ce}}(A;\mathbf{B})$ represents cross-entropy loss where $A$ is the correct label and $\mathbf{B}$ is the set of all candidate labels. $\beta$ is a hyperparameter that adjusts the relative weights of the two loss items. We found $\beta=0.1$ works the best through our hyperparameter sweep experiments.

% Assuming the logit for the other class is denoted as $l_{\text{other}}$, the encoded image embedding is $e_{\text{ft}}^I$, and the text embedding for target class $y_t$ is $e_{y_t}$, then
% \begin{equation}
% \label{eq:p_other}
%     p_{\text{other}} = \frac{\exp({l_{\text{other}}})}{\sum_{y_t}^{\mathcal{C}_t} \exp({100 * e_{\text{ft}}^I e_{y_t}}) + \exp({l_{\text{other}}})}.
% \end{equation}

% We are inspired by the open-world recognition literature~\cite{??} to introduce the prediction of an ``other'' class. If a sample is assigned to the other class, it means that the sample is OOD. The success of predicting an OOD sample as the other class is mainly practiced by drawing negative samples as learning materials to help the model discern the boundary between the ``other'' class and all other classes. 


% Then the $\alpha$ is calculated by:
% \begin{equation}
%     \alpha = (1-\sigma p_{\text{other}})(\frac{p_{\text{ft}}}{p_{\text{ft}} + p_{\text{zs}}  + \epsilon}).
% \end{equation}
% Here, $\epsilon=1e^{-6}$ is used to avoid cases where the divisor is 0.  

% Then the final probability of our system is:
% \begin{equation}
%     p_{\text{out}} = \alpha p_e + (1-\alpha) p_z,
% \end{equation}
% here $p_e=\text{softmax}(100 * e_{\text{ft}}^I e_{y_t})$ and $p_z = \text{softmax}(100 * e_{\text{zs}}^I e_{y_t})$. $e_{\text{zs}}^I$ is the encoded image embedding from the zero-shot transformer block.



\subsection{Storage efficiency and privacy}

Partial tuning of our models requires either storing each image or storing the features (or tokens) that feed into the tuned portion of the model. Storing images is disadvantageous in terms of privacy, storage of the full model and images, and in requiring full processing of the images at each iteration. Storing features alleviates some of these problems, but storing all features at some layer requires even more storage than compressed images.  Therefore, we investigate how to compress the training features, aiming to increase storage and computational efficiency while maintaining training effectiveness. The compressed features also provide more privacy than storing original images, though we do not investigate how well the images can be recovered from compressed features.

Well trained networks learn data-efficient representations that are difficult to compress. Indeed, if we try to compress feature vectors with VQ-VAE~\cite{vqvae} or PCA~\cite{pca} trained on a dataset, we are not able to achieve any meaningful compression without great loss in training performance. The features within {\em each image}, however, contain many redundancies. We, therefore, compute PCA vectors on the features in each image and store those vectors along with the coefficients of each feature vector. Further, not all features are equally important for prediction. We, therefore, train a weighted PCA, weighted by attention between each token and the CLS token. Finally, we can compress further by storing min/max floating point values for each vector and for the coefficients and quantizing them to 8-bit or 16-bit unsigned integers. See the supplemental material for details.  By storing only five PCA vectors and their coefficients this way, we can reduce the storage of fifty 768-dim patch tokens from 153K bytes to 4K bytes with less than 1\% difference in prediction accuracy. 

==> sec/memory_compression_text.tex <==
We perform data compression on our intermediate representations output from the $\mathbf{M}_{\text{base}}$ block in a per-instance manner. Every image will be output as a $50 \times 768$ dimensional embedding from $\mathbf{M}_{\text{base}}$. We explicitly choose the number of components for the embeddings to be compressed to, which we denote as $n$. $n$ is shared among all the embeddings, so after compression, for each embedding, we will get the principle components of size $n \times 768$, along with its coefficients of size $50 \times n$, and the mean value of size $768$ which is used to center the data.

Therefore, PCA will give us a compression rate of:
\begin{equation}
    \label{eq:pca_compression_rate}
    R_{base} = \frac{50 \times 768}{50 \times n + n \times 768 + 768}
\end{equation}
We use $R_{base}$ to denote the base case compression rate when only incorporating PCA.

We further leverage the fact that each token in the embedding has different contribution towards the prediction accuracy. Thus we want to weight our embeddings in order to emphasis on the most influential tokens. We achieve this by using the attention between each token and the CLS token. We obtain the attention from the last attention layer in $\mathbf{M}_{\text{base}}$ and perform softmax across the them to get the weight for each token. By directly multiplying each token with its weight, we get the weighted embedding to be fed into PCA and thus we can get the principle components and means. In order to be able to recover the original embedding, we still need the $50 \times n$ dimensional coefficients. We obtain the coefficients as
\begin{equation}
    \label{eq:calculate_coefficient}
    C = MatMul((E - m), inv(P)) 
\end{equation}
$C$ is the coefficients we want to obtain, $E$ is the original embedding without weighting, $m$ and $P$ are the means and principle components we get from the weighted embedding. For $inv(P)$, we take the pseudo inverse of the principle components, and for $MatMul$, we do the matrix multiplication between the two terms. The compression rate calculation for weighted PCA follows the same equation as $R_{base}$, but by using weighted PCA, the most important tokens can be better represented with few components; thus, we can maintain similar prediction accuracy with a smaller $n$.


We can further decrease our memory footprint by performing unit8 quantization. For each vector in principle components, coefficients, and means, we will store the min/max floating point values and then cast each element in the vector into a 8-bit unsigned integer. By storing the 32-bit floating point value as 8-bit unsigned integer, we can further get a 4 times decrease in memory usage comparing to the PCA-compressed embeddings. The detailed calculation is as follow:
\begin{equation}
    \label{eq:int_quantize}
    Int(v_i) = Round(\frac{v_i-v_{min}}{v_{max} - v_{min}} \times 255)
\end{equation}
$v_i$ is the $ith$ element in the vector $v$, which may come from principle components, coefficients or be the mean vector. $v_{max}$ and $v_{min}$ is the maximum and minimum floating point value in $v$.

==> sec/prompt_tuning_section.tex <==
\subsection{Using visual prompts}

\input{figures/latex/prompt_tuning}
As the practice of prompt tuning to improve LLMs' performance on certain tasks~\cite{??}, prompt tuning is also effective for vision tasks when using transformers as backbones~\cite{jia_2022_VPT,wang_2022_CVPR_l2p}.
Since visual prompts are easily extensible and the original parameters of the transformer backbone are fixed during training, prompt-tuning naturally fits the goal of continual learning to improve on target tasks without losing generality to old tasks. Therefore, a large body of works explore methods to leverage visual prompt tuning effectively for continual learning. To understand the pros and cons of prompt-tuning for our system, we create a variation of our system using learnable visual prompts instead of a tuned decoder. This variation (AnytimeCL-VPT) also contains a dual system producing two outputs with one from applying the whole network without using visual prompts and the other one from appending visual prompts to certain or all layers of the transformer backbone. We use the same weighting method to balance the two outputs. 

Following VPT~\cite{jia_2022_VPT}, we also study both a shallow version and a deep version of AnytimeCL-VPT. The shallow version only applies some number of prompts on the first transformer block, whereas the deep one applies prompts to the last transformer block. Note that finding which layers to add visual prompts can potentially improve performance further, but is out of scope of this study. We also vary the number of visual prompts to show whether using more prompts is generally better. We perform this set of ablation experiments under the union data incremental scenario. As a sanity check and hyperparameter selection, we run batch training experiments on CIFAR100. On the comparison to partial-tuning the last transformer block whose accuracy is 82.1\% on the validation set, the shallow version achieves 82.7\% and the deep version obtains 73.8\%. 

Results are shown in Fig.~\ref{fig:prompt_tuning}. Apparently, using shallow prompts is better than using deep prompts. However, the shallow version is significantly slower than the deep version, because the shallow one needs to pass through the entire transformer, whereas the deep one only needs to pass through the last transformer block once the intermediate representation of the input sample is stored. Another take-away message from the plot is that using more prompts is not always better, especially for the shallow case, where using 50 prompts generally beats using more. 

Note that the default version of AnytimeCL is significantly better than the prompt tuning version, possibly because the varying data distribution continually disturbs the optimization of learnable prompts. However, the problem can be partially treated by implementing retrieval of suitable prompts for the input sample~\cite{wang_2022_CVPR_l2p}. In the long run, visual prompt tuning still shows great potentials in offering alternative methods for weight-based tuning.

==> tables/ablation_on_partial_finetuning.tex <==
\begin{table}[ht]
\centering
\caption{Ablation study on fine-tuning last transformer block ({\em trans. blk}) of the encoder and the label classifier ({\em label cls.}) under task incremental learning.}
\label{tab:performance_metrics}
\scalebox{0.65}{
\begin{tabularx}{1.5\textwidth}{*{10}{X}}
\toprule
 {\em trans. blk.} & {\em label cls.} & CIFAR100 & SUN397 & EuroSAT & Pets & Flowers & Aircraft & Cars & Food \\ 
\midrule
No & No & 60.2 & 60.2 & 60.2 & 60.2 & 60.2 & 60.2 & 60.2 & 60.2 \\
No & Yes & xx & xx & xx & xx & xx & xx & xx & xx \\
Yes & Yes & 61.5 & 64.7 & 70.8 & 70.4 & 71.5 & 74.5 & 76.4 & 78.9 \\
Yes & No & 62.8 & 64.9 & 71.0 & 71.8 & 74.6 & 77.5 & 80.6 & 82.1 \\ \bottomrule
\end{tabularx}
}
\end{table}


==> tables/ablation_tables.tex <==
\begin{figure}[htb]
    \centering
    % First minipage for the first small table
    \begin{minipage}{0.3\textwidth}
        \centering
        \captionof{table}{Ablation results on the EMA decay parameter and 1-NN cross validation}
        \label{tab:ema_decay_ablation}
        \scalebox{0.5}{
        \begin{tabular}{|l|c|c|}
            \hline
            \textbf{Est. Method} & \textbf{EMA decay} & \textbf{Accuracy} \\ \hline
\multirow{6}{*}{EMA} & 0.1 & 81.50 \\ 
                            & 0.3 & 81.69 \\ 
                            & 0.5 & 81.74 \\ 
                            & 0.7 & 81.78 \\  
                            & 0.9 & 81.81 \\ 
                            & 0.99 & 81.82 \\ \hline
1-NN cross val. & - & 81.73 \\ \hline
        \end{tabular}
        }
    \end{minipage}
    \hfill % Adds horizontal space between the minipages
    % Second minipage for the second small table
    \begin{minipage}{0.3\textwidth}
        \centering
        \captionof{table}{Results of AnytimeCL online in different node capacities.}
        \label{tab:second_small_table}
        \scalebox{0.5}{
        \begin{tabular}{|l|c|}
        \hline
        \textbf{Node capacity} & \textbf{Accuracy} \\
        \hline
        50k & 79.39 \\
        100k & 82.08 \\
        150k & 82.06 \\
        200k & 79.96 \\
        Infinite & 81.10 \\ 
        \hline
        \end{tabular}
        }
    \end{minipage}
    \hfill % Adds horizontal space between the minipages
    \begin{minipage}{0.3\textwidth}
        \centering
        \captionof{table}{Ablation results on the impact of batch size. Experiments are done by online learning on the union of all target tasks. Results are reported as the average accuracy of all target tasks.}
        \label{tab:second_small_table}
        \scalebox{0.5}{
\begin{tabular}{|l|l|c|}
\toprule
\textbf{bs.} & \textbf{lr.} &  \textbf{Acc.} \\
\midrule
256 & 5e-4 & 82.2 \\
64 & 1.25e-5 & 81.9 \\
32 & 6.25e-6 & 81.8 \\
16 & 3.12e-6 & 81.2 \\
8 & 1.56e-6 & 80.7 \\
\bottomrule
\end{tabular}
}
    \end{minipage}
\end{figure}


==> tables/dataset_n_components.tex <==
\begin{table}
\centering
\scalebox{1}{
\begin{tabular}{lcc}
\toprule
No. components &  FT Accuracy & KB/example\\
\midrule
100 & 74.9 & 20.1\\
200 & 76.3 & 40.2\\
300 & 77.1 & 60.1\\
400 & 77.4 &  80.2\\
500 & 77.6 &  100.3\\
\bottomrule
\end{tabular}
}
\caption{Dataset-wide fine-tuning accuracy with different components. 
% \zhen{Also, can we include KB/example here?}
\label{tab:dataset_different_components}}
\end{table}

==> tables/decay_multiplier.tex <==
\begin{table}
\centering
\caption{Performance of different $\xi$ in union data incremental learning and class incremental learning scenarios. All experiments adopt the online training setting. Result in the table is the average accuracy across all target tasks after receiving all data.}
\begin{tabular}{lcc}
\toprule
{Decay multiplier $\xi$} & {Data-Inc. Acc.} & {Class-Inc. Acc.}\\
\midrule
1.00 & 81.5 & 82.0 \\
0.99 & 81.5 & 82.1 \\
0.95 & 81.8 & 81.3 \\
0.90 & 81.7 & 80.2 \\
0.85 & 81.4 & 80.5 \\
0.80 & 81.6 & 81.0 \\
0.75 & 81.6 & 81.0 \\
0.70 & 81.6 & 81.7 \\
\bottomrule
\end{tabular}
\label{tab:decay_multiplier}
\end{table}

==> tables/ensemble_classifiers.tex <==
\begin{table}[ht]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Stage I} & \multicolumn{2}{c}{Stage II} & \multicolumn{2}{c}{Stage III} & \multicolumn{2}{c}{Stage IV} & \multicolumn{2}{c}{Stage V} & \multicolumn{2}{c}{Stage VI} & \multicolumn{2}{c}{Stage VII} & \multicolumn{2}{c}{Stage VIII} \\ \cline{2-17}
 & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot & Target & Zero-shot \\ \hline
\tp\ w/o ensem. cls. & 60.3 & 53.6 & 63.0 & 53.5 & 70.3 & 53.8 & 70.3 & 53.7 & 70.0 & 53.8 & 71.9 & 53.8 & 74.8 & 53.8 & 74.4 & 53.8  \\ \hline
\tp\ & 61.7 & 53.9 & 63.2 & 53.8 & 70.6 & 53.9 & 70.6 & 53.8 & 70.6 & 53.8 & 72.5 & 53.8 & 75.5 & 53.8 & 75.3 & 53.9 \\  \hline
\end{tabular}
\end{adjustbox}
\caption{Accuracies of \czs\ and \tp\ on target and zero-shot tasks with pretrained image encoders of different capacities.}
\label{tab:ensemble_classifiers}
\end{table}

==> tables/loss_weight.tex <==
\begin{table}
\centering
\caption{Performance of various $\beta$ using online learning and offline learning. For online accuracy, the result is the average of accuracy on all target tasks after all data is received (union data incremental). For offline accuracy, the result is obtained by training the model for 32 epochs on the union of all target tasks.}
\begin{tabular}{lcc}
\toprule
Loss weight $\beta$ & {Online Acc.}  & Offline Acc. \\
\midrule
0.0 & 80.9 & 82.2 \\
0.1 & 81.5 & 83.0 \\
0.2 & 81.5 & 82.9 \\
0.3 & 81.5 & 82.9 \\
0.4 & 81.6 & 82.9 \\
0.5 & 81.6 & 82.9 \\
0.6 & 81.6 & 82.8 \\
0.7 & 81.6 & 82.6 \\
0.8 & 81.5 & 82.3 \\
0.9 & 81.6 & 82.2 \\
1.0 & 81.5 & 82.2 \\
% \rowcolor{yellow} 0.1 & \textbf{82.517} \\
\bottomrule
\end{tabular}
\label{tab:loss_weight}
\end{table}


==> tables/new_results_compared_to_zscl.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
52.45 & 87.90 & 68.22 & 45.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
\hline
52.48 & 96.89 & 68.22 & 45.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
\hline
52.48 & 96.83 & 81.95 & 45.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
\hline
52.42 & 96.83 & 81.97 & 70.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
\hline
52.42 & 90.03 & 82.01 & 67.07 & 95.78 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
\hline
52.48 & 91.42 & 81.84 & 66.91 & 95.78 & 55.29 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
\hline
52.48 & 91.01 & 81.95 & 67.39 & 95.76 & 65.10 & 92.23 & 59.45 & 89.07 & 64.61 & 64.05 \\
\hline
52.09 & 93.89 & 82.05 & 69.79 & 94.30 & 95.69 & 92.25 & 98.58 & 89.07 & 64.61 & 64.05 \\
\hline
52.63 & 95.16 & 82.00 & 70.16 & 95.57 & 95.69 & 92.24 & 98.60 & 92.86 & 64.61 & 64.05 \\
\hline
52.60 & 95.28 & 81.91 & 68.09 & 94.24 & 95.59 & 92.24 & 98.59 & 93.19 & 86.27 & 64.05 \\
\hline
52.42 & 92.97 & 81.97 & 63.35 & 95.59 & 92.55 & 92.24 & 98.58 & 93.13 & 86.17 & 81.84 \\
\hline
\end{tabular}


\begin{table*}
\begin{tabular}{rrrrrrrrrrr}
\toprule
   0  &    1  &    2  &    3  &    4  &    5  &    6  &    7  &    8  &    9  &    10 \\
\midrule
45.18 & 87.90 & 68.22 & 45.32 & 54.49 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
49.56 & 96.89 & 68.22 & 45.32 & 54.49 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
50.17 & 97.06 & 81.07 & 45.32 & 54.49 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
50.38 & 96.83 & 81.34 & 58.40 & 54.49 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
48.66 & 96.77 & 81.96 & 64.57 & 54.49 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
50.56 & 96.60 & 81.98 & 65.05 & 54.49 & 81.86 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
50.62 & 96.54 & 81.89 & 64.63 & 54.49 & 86.18 & 91.90 & 59.45 & 89.07 & 64.61 & 64.05 \\
49.20 & 96.49 & 81.33 & 65.16 & 54.49 & 86.37 & 92.05 & 59.45 & 89.07 & 64.61 & 64.05 \\
51.52 & 96.26 & 81.79 & 64.20 & 54.49 & 87.35 & 92.19 & 59.45 & 90.76 & 64.61 & 64.05 \\
50.59 & 96.60 & 81.73 & 65.32 & 54.49 & 87.94 & 92.05 & 59.45 & 90.90 & 76.96 & 64.05 \\
 0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/results_under_zscl_setting.tex <==
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lcccccccccccc@{}}
    \toprule
    \noalign{\smallskip}
     & \rotatebox{90}{Aircraft} & \rotatebox{90}{Caltech101} & \rotatebox{90}{CIFAR100} & \rotatebox{90}{DTD} & \rotatebox{90}{EuroSAT} & \rotatebox{90}{Flowers} & \rotatebox{90}{Food} & \rotatebox{90}{MNIST} & \rotatebox{90}{OxfordPet} & \rotatebox{90}{Cars} & \rotatebox{90}{SUN397} & \\ 
    \noalign{\smallskip} 
    \hline \hline \noalign{\smallskip}
    Transfer &  & 87.90 & 68.22 & 45.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 & \cellcolor{green!40}{69.3} \\
    \midrule
    Aircraft & 52.45 & 87.90 & 68.22 & 45.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05\\
    Caltech101 & 52.48 & 96.89 & 68.22 & 45.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05\\
    CIFAR100 & 52.48 & 96.89 & 68.22 & 45.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05\\
    DTD & 52.42 & 96.83 & 81.98 & 70.32 & 54.61 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05\\
    EuroSAT & 52.45 & 89.92 & 81.99 & 66.65 & 95.74 & 71.08 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05 \\
    Flowers & 52.51 & 90.55 & 81.93 & 66.44 & 95.74 & 54.12 & 88.86 & 59.45 & 89.07 & 64.61 & 64.05\\
    Food & 52.48 & 90.78 & 81.94 & 67.23 & 95.78 & 65.49 & 92.25 & 59.45 & 89.07 & 64.61 & 64.05\\
    MNIST & 52.09 & 93.95 & 81.96 & 69.73 & 94.33 & 95.69 & 92.27 & 98.59 & 89.07 & 64.61 & 64.05 \\
    OxfordPet & 52.63 & 95.10 & 82.05 & 70.05 & 95.63 & 95.69 & 92.29 & 98.58 & 92.91 & 64.61 & 64.05\\
    Cars & 52.54 & 95.22 & 81.94 & 67.98 & 94.15 & 95.59 & 92.29 & 98.58 & 93.02 & 86.27 & 64.05\\
    SUN397 & 52.48 & 95.56 & 81.94 & 66.91 & 95.59 & 95.59 & 92.21 & 98.60 & 93.19 & 86.15 & 81.76 & \cellcolor{orange!40}{85.5} \\
    \midrule
    Avg. & 52.45 & 93.59 & 79.47 & 61.93 & 80.49 & 77.96 & 90.40 & 73.68 & 90.15 & 68.53 & 65.66 & \cellcolor{blue!30}{75.9}\\
    \bottomrule
    \end{tabular}
}
\caption{Accuracy (\%) of our \tp\ (50k) model on the MTIL benchmark with order-I. Each row represents the performance on every dataset of the model trained after the corresponding task. Transfer, \cellcolor{blue!30}{Avg.}, and Last metrics are shown in color. We follow the same table arrangement as in ZSCL~\cite{ZSCL}.}
\label{tab:results_under_zscl}
\end{table*}

==> tables/sun_compression.tex <==
\begin{table}
\centering
\scalebox{0.67}{
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Compression} & \textbf{KB/example} & \textbf{ms/batch} & \textbf{FT Accuracy} \\
\hline
Full image & 150.5 & 612.5 & 77.3 \\
Full features & 153.6 & 20.5 & 77.3 \\
VQ & 0.2 & 3.3 & 65.1 \\
Dataset-wide PCA (200 components) & 40.2 & 5.9 & 75.8 \\
Per-instance PCA (5 components) & 19.4 & 5.8 & 71.3 \\
+ CLS-weight (5 components) & 19.4 & 6.1 & 77.6 \\
+ int-quantization (5 components) & 5.3 & 12.0 & 77.4 \\
\hline
\end{tabular}
}
\caption{Comparison of different compression methods in terms of memory usage, processing speed, and test accuracy. \zhen{Isn't it strange that the Full Image and Full feature have inferior results to compressed representations?}}
\label{tab:sun_compression}
\end{table}

==> tables/supp_comparizon_to_zscl.tex <==
\begin{minipage}{\linewidth}
\centering
\begin{adjustbox}{width=.8\textwidth}
\begin{tabular}{|l|cc|cc|cc|}
\hline
\textbf{Method} & \textbf{Transfer} & $\triangle$ & \textbf{Avg.} & $\triangle$ & \textbf{Last}  & $\triangle$\\
\hline
CLIP Zero-shot & 69.4 & 0.0 & 65.3 & 0.0 & 65.3 & 0.0 \\ \hline
LwF~\cite{LwF} & 56.9 & \red{-12.5} & 64.7 & \red{-0.6} & 74.6 & \green{+9.3} \\
iCaRL~\cite{iCaRL} & 50.4 & \red{-19.0} & 65.7 & \green{+0.4} & 80.1 & \green{+14.8} \\
WiSE-FT~\cite{WiSE-FT} & 52.3 & \red{-17.1} & 60.7 & \red{-4.6} & 77.7 & \green{+12.4} \\
ZSCL~\cite{ZSCL}   & 68.1 & \red{-1.3} & 75.4 & \green{+10.1} & 83.6 & \green{+18.3} \\ \hline
KNN & 69.3 & {\red{-0.1}} & 72.7 & {\green{+7.4}} & 78.4 & {\green{+13.1}} \\
\lp\ & {69.3} & {\red{-0.1}} & {77.1} & {\green{+11.8}} & {86.0} & {\green{+20.7}} \\
\tp\ (50k) & {69.3} & {\red{-0.1}} & {75.9} & {\green{+10.6}} & {85.5} & {\green{+20.2}} \\ \hline 
\end{tabular}
\end{adjustbox}
\captionof{table}{Comparison of different methods on MTIL in Order I from ZSCL~\cite{ZSCL}. KNN, \lp\ , and \tp\ (50k) are complementary methods with AIM-Emb as the fusing approach. }
\label{tab:supp_comparison_to_zscl}
\end{minipage}

==> tables/tree_models.tex <==
\begin{table}
\centering
\scalebox{0.9}{
\begin{tabular}{|l|c|c|}
\hline
\textbf{Model} & \textbf{Wake} & \textbf{Sleep} \\
\hline
AnytimeCL (tree 50k) & 80.9 & 76.2 \\
AnytimeCL (tree 100k) & 82.7 & 83.7 \\
AnytimeCL (tree 150k) & 82.9 & 83.6 \\
AnytimeCL (tree 200k) & 80.9 & 81.7 \\
AnytimeCL (single node) & 82.2 & 82.6 \\ 
\hline
\end{tabular}
}
\caption{Results of AnytimeCL in different node capacities.   }
\label{tab:tree_models}
\end{table}



==> tables/wake_batch_size_ablation.tex <==
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{llc}
\toprule
\textbf{Wake Batch Size} & \textbf{Wake Learning Rate} &  \textbf{Wake Accuracy} \\
\midrule
256 & 5e-4 & 82.2 \\
64 & 1.25e-5 & 81.9 \\
32 & 6.25e-6 & 81.8 \\
16 & 3.12e-6 & 81.2 \\
8 & 1.56e-6 & 80.7 \\
\bottomrule
\end{tabular}
}
\caption{Ablation results on the impact of batch size. Experiments are done by online learning on the union of all target tasks. Results are reported as the average accuracy of all target tasks.}
\label{tab:wake_batch_size_ablation}
\end{table}
